Model studies of the chiral and deconfinement transitions in QCD

The Doctoral thesis of William Naylor. Gives the background of the three papers included, specifically introducing both the quark meson model and the NJL model, the basic formalism of thermal field theory, and functional renormalization group (including some details on numerically solving the FRG equation for the QM model).

==> 02_Chapters/abstract.tex <==
\chapter*{Abstract}

Abstract to go here.

%  This thesis is devoted to the theoretical study of spin-orbit-induced transport in diffusive normal metals and superconductors. The spin-orbit interaction plays a vital role in the aspiring field of spintronics, which aims to utilize the electron spin with the ambition to enable a new generation of efficient and powerful electronic devices. It provides a link between the spin and charge degrees of freedom, couples spin currents of different polarizations, and leads to the dephasing of spin information.
%  
%  We elucidate the nature of the spin swapping effect, where the spin polarization and the direction of flow are interchanged due to spin-orbit coupling, and demonstrate that an intrinsic analog to the previously predicted extrinsic spin swapping effect can be induced by Rashba spin-orbit coupling in two-dimensional diffusive metals. Unlike its extrinsic counterpart, intrinsic spin swapping is a strong effect and results in a nontrivial relation between the injected spin flow and the spin polarization. Moreover, a long-range spin swapping effect takes place in narrow strips with intrinsic spin-orbit coupling.
%  
%  Rich and interesting physics emerge when the useful properties of superconductors are combined with spin generation and manipulation. We study in detail spin relaxation due to magnetic impurity scattering and spin-orbit coupling, skew scattering, the side-jump mechanism, and the spin swapping effect. Employing the quasiclassical theory of superconductivity, we derive kinetic equations describing the transport of spin, charge, and energy in diffusive superconductors, and investigate how the various mechanisms are influenced by superconducting correlations. We find that the spin Hall angle is renormalized by the superconducting density of states and that the spin swapping constant is renormalized implicitly through generalized diffusion coefficients.
%  
%  Additionally, we consider an inverse spin Hall effect occurring due to the interplay between Rashba spin-orbit coupling and Zeeman fields in S$|$N$|$S Josephson junctions in thermal equilibrium. This combination induces an effective vector potential in the normal conductor and gives rise to a supercurrent, in analogy to the Meissner effect. Spin-orbit coupling also diminishes the depairing effects of strong Zeeman fields and leads to a long-range propagation of $\pm 1$ triplet components on the scale of the spin-orbit precession length, providing a link between the two superconducting terminals.
%  
%  It is the aim of this thesis to contribute to a fundamental understanding of the physical properties of nanoscaled condensed matter systems, obtain results that may inspire further research, and thereby aid the development of novel and improved technologies in the promising field of spintronics.

==> 02_Chapters/conclusion.tex <==
\chapter{Concluding remarks}
\label{cha:conclusion}

we have done something
  
  
%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
%
\section{Summary}
\label{sec:summary}

asdf


% //////////////////////////////////////////////////////////////////////////////////////////////////////////////


%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
%
\section{Outlook}
\label{sec:outlook}

asdf


% //////////////////////////////////////////////////////////////////////////////////////////////////////////////


==> 02_Chapters/symmetries.tex <==
\chapter{Symmetries and their breaking in QCD}
\label{cha:symmetries}

We will deal repeatedly with the breaking and restoration of various symmetries 

The most general starting point in building a relativistic quantum theory of strongly interacting matter is the Poincar{\'e} group. This group is the non-abelian Lie group made up of three distict operations:
\begin{itemize}
\item Translations, i.e.\ 
\item Rotations, i.e.\ 
\item Boosts, i.e.\ 
\end{itemize}
We then wish to build our theory 

The most obvious representations of this group, with which we will obviously want to construct our theory, 

%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
%
\section{Thermal field theory}
\label{sec:thermal_field_theory}


%  such that the currents of Eqs.~\eqref{eq:current_definition} in the quasiclassical approximation are given by
%  % -------------------------------------------------------
%  % Currents in Quasiclassics
%  \begin{subequations}
%  \label{eq:current_quasi}
%  \begin{align}
%  \label{eq:current_quasi_particle}
%   J_i(\vect{R})
%   &=
%   -
%   \frac{N_0}{4}
%   \int \diffint{\epsilon}{} \operatorname{Tr}\big[ \tauhat{3} \hat{\jmath}_i(\vect{R}, \epsilon) \big]
%  \\
%  \intertext{and}
%  \label{eq:current_quasi_spin}
%   J_{ij}(\vect{R})
%   &=
%   -
%   \frac{N_0}{4}
%   \int \diffint{\epsilon}{} \operatorname{Tr}\big[ \tauhat{3} \hat{\alpha}_j \hat{\jmath}_i(\vect{R}, \epsilon) \big]
%   .
%  \end{align}
%  \end{subequations}
%  % - - - - - - - - - - - - - - - - - - - - - - - - - - - -
%  In addition to the aforementioned corrections to Eqs.~\eqref{eq:usadel_anisotropic} and~\eqref{eq:usadel} due to magnetic impurities and spin-orbit coupling, the velocity operator~\eqref{eq:velocity_definition} acquires anomalous contributions in the presence of spin-orbit coupling. These shall be discussed in Chapters~\ref{cha:mechanisms} and~\ref{cha:extrinsic_soc_superconductors}.
%  
%  
%% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
%
%
%
%% ----------------------------------------------------------------------------------------------------------------------------------
%% 
%% Boundary Conditions
%\subsection{Boundary Conditions}
%
%  The quasiclassical approximation, which assumes that relevant quantities vary on length scales much larger than the Fermi wavelength, naturally breaks down in the vicinity of interfaces. However, the quasiclassical Green's functions describing two distinct regions $1$ and $2$ can be connected across an intermediate boundary surface with the aid of scattering theory. In the limit of a low-transparency interface perpendicular to the $x$ direction, the boundary condition reads~\cite{Kuprianov1988,Lambert1998}
%  % -------------------------------------------------------
%  \begin{equation}
%  \label{eq:greens_boundary}
%   2 \sigma
%   \check{g}_\text{s}^{(2)} \nabla_x \check{g}_\text{s}^{(2)}
%   =
%   G_\text{T}
%   \big[
%    \check{g}_\text{s}^{(2)}
%    ,
%    \check{g}_\text{s}^{(1)}
%   \big]_{-}
%   ,
%  \end{equation}
%  % - - - - - - - - - - - - - - - - - - - - - - - - - - - -
%  where $\sigma = 2 e^2 N_0 D$ is the conductivity, $G_\text{T} = e^2 N_0 v_\text{F} \langle {e_p}_x T({e_p}_x)/R({e_p}_x)\rangle_\text{F}$ is the interface conductance, and $T$ and $R$ are the interface transmission and reflection coefficients, respectively.
%  
%  
%% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
%
%  
%% //////////////////////////////////////////////////////////////////////////////////////////////////////////////////////////////////
%
%
%
%%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
%%
%%\section{The Normal Limit}
%%\label{sec:fundamentals_normal}



